Trade-offs in Medical LLM Adaptation: An Empirical Study in French QA

The development of large language models (LLMs) has led to an increased focus on their adaptation to specialized domains and languages, yet the effectiveness of domain adaptation strategies remains unclear. We present a study of medical domain adaptation using French medical question-answering (QA) as a case study. We compare continual pretraining (CPT), supervised fine-tuning (SFT), and their combination across three model families, multiple sizes, and three initialization types, explicitly disentangling adaptation effects from base model choice. We evaluate both multiple-choice (MCQA) and open-ended QA (OEQA) under greedy and constrained decoding using automatic metrics and LLM-as-a-Judge evaluation. For MCQA, CPT+SFT most often achieves the best scores, but gains over SFT are small and frequently not statistically significant, making SFT a strong and cost-effective default. For OEQA, CPT consistently improves overlap-based metrics, while SFT often degrades generation quality; instruction tuning and CPT+SFT are preferred by LLM-based evaluation. Cross-lingual experiments further show effective transfer from French adaptation to English benchmarks. Overall, we provide practical guidelines for selecting adaptation strategies under computational constraints.

==> correlation-judges.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[H]
\centering
\setlength{\extrarowheight}{2pt}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llll}
\cline{3-4}
 & \textbf{} & {\textbf{Pearson\_r}} & {\textbf{F1}} \\ \hline
\multirow{5}{*}{\begin{turn}{90}\textbf{Judges}\end{turn}} & \textbf{GPT5.1} & 38,27 & 45,07 \\ \cdashline{2-4}
 & \textbf{GEMINI-2.5-PRO} & 38,81 & 52,59 \\ \cdashline{2-4}
 & \textbf{QWEN-80b} & \textbf{44,77} & 60,00 \\ \cdashline{2-4}
 & \textbf{MEDGEMMA-27B} & 40,67 & \textbf{60,50} \\ \cdashline{2-4}
 & \textbf{M-PROMETHEUS} & 34,88 & 48,56 \\ \hline
\multirow{5}{*}{\begin{turn}{90}\textbf{Metrics}\end{turn}} & \textbf{ROUGE-L} & 25,40 & - \\ \cdashline{2-4}
 & \textbf{METEOR} & 25.04 & - \\ \cdashline{2-4}
 & \textbf{BLEU} & 17,16 & - \\ \cdashline{2-4}
 & \textbf{BERTScore\_F1} & 14,88 & - \\ \hline 
\end{tabular}%
}
\caption{Agreement between human judgments and automatic evaluation methods for OEQA.}
\label{tab:judges-corr}
\end{table}

==> en-eval-results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\centering
\resizebox{0.6 \columnwidth}{!}{%
\begin{tabular}{cccc}
\hline
\textbf{Model Type} & \textbf{Strategy} & \textit{\textbf{QCMU-FR}} & \textit{\textbf{QCMU-EN}} \\ \hline
\multicolumn{4}{c}{\cellcolor[HTML]{CFE2F3}\textit{\textbf{Gemma-4B}}} \\ \hline
 & \textbf{Base} & 26,63 & \textbf{41,22} \\  
 & {\color[HTML]{0000FF} \textbf{CPT}} & 25,60 & \textbf{40,10} \\  
 & {\color[HTML]{6AA84F} \textbf{SFT}} & 32,82 & \textbf{51,60} \\  
\multirow{-4}{*}{\textbf{GENERAL}} & {\color[HTML]{FF0000} \textbf{CPT+SFT}} & 32,73 & \textbf{51,42} \\ \hline
 & \textbf{Base} & 29,76 & \textbf{47,94} \\  
 & {\color[HTML]{0000FF} \textbf{CPT}} & \textbf{24,28} & 23,43 \\  
 & {\color[HTML]{6AA84F} \textbf{SFT}} & 32,46 & \textbf{48,74} \\  
\multirow{-4}{*}{\textbf{INSTRUCT}} & {\color[HTML]{FF0000} \textbf{CPT+SFT}} & 30,38 & \textbf{39,17} \\ \hline
 & \textbf{Base} & 26,43 & \textbf{32,47} \\  
 & {\color[HTML]{0000FF} \textbf{CPT}} & \textbf{24,71} & 23,85 \\  
 & {\color[HTML]{6AA84F} \textbf{SFT}} & 30,77 & \textbf{45,03} \\  
\multirow{-4}{*}{\textbf{MEDICAL}} & {\color[HTML]{FF0000} \textbf{CPT+SFT}} & 30,50 & \textbf{40,14} \\ \hline
\multicolumn{4}{c}{\cellcolor[HTML]{CFE2F3}\textit{\textbf{Mistral-7B}}} \\ \hline
 & \textbf{Base} & \textbf{28,96} & 26,15 \\  
 & {\color[HTML]{0000FF} \textbf{CPT}} & \textbf{27,15} & 25,20 \\  
 & {\color[HTML]{6AA84F} \textbf{SFT}} & \textbf{32,98} & 27,00 \\  
\multirow{-4}{*}{\textbf{GENERAL}} & {\color[HTML]{FF0000} \textbf{CPT+SFT}} & \textbf{32,22} & 27,39 \\ \hline
 & \textbf{Base} & \textbf{25,51} & 25,10 \\  
 & {\color[HTML]{0000FF} \textbf{CPT}} & \textbf{29,69} & 25,51 \\  
 & {\color[HTML]{6AA84F} \textbf{SFT}} & \textbf{31,74} & 26,38 \\  
\multirow{-4}{*}{\textbf{INSTRUCT}} & {\color[HTML]{FF0000} \textbf{CPT+SFT}} & \textbf{30,11} & 25,21 \\ \hline
 & \textbf{Base} & \textbf{26,88} & 25,69 \\  
 & {\color[HTML]{0000FF} \textbf{CPT}} & \textbf{25,49} & 24,32 \\  
 & {\color[HTML]{6AA84F} \textbf{SFT}} & \textbf{31,64} & 26,28 \\  
\multirow{-4}{*}{\textbf{MEDICAL}} & {\color[HTML]{FF0000} \textbf{CPT+SFT}} & \textbf{32,33} & 26,90 \\ \hline

\multicolumn{4}{c}{\cellcolor[HTML]{CFE2F3}\textit{\textbf{Llama-7B}}} \\ \hline
 & \textbf{Base} & \textbf{25,48} & 25,17 \\  
 & {\color[HTML]{0000FF} \textbf{CPT}} & 25,27 & \textbf{28,56} \\  
 & {\color[HTML]{6AA84F} \textbf{SFT}} & 28,61 & \textbf{32,87} \\  
\multirow{-4}{*}{\textbf{GENERAL}} & {\color[HTML]{FF0000} \textbf{CPT+SFT}} & 29,77 & \textbf{39,25} \\ \hline
 & \textbf{Base} & \textbf{24,34} & 23,44 \\  
 & {\color[HTML]{0000FF} \textbf{CPT}} & \textbf{24,29} & 23,49 \\  
 & {\color[HTML]{6AA84F} \textbf{SFT}} & 29,58 & \textbf{38,73} \\  
\multirow{-4}{*}{\textbf{INSTRUCT}} & {\color[HTML]{FF0000} \textbf{CPT+SFT}} & \textbf{24,54} & 23,45 \\ \hline
 & \textbf{Base} & \textbf{24,19} & 23,68 \\  
 & {\color[HTML]{0000FF} \textbf{CPT}} & \textbf{25,14} & 24,96 \\  
 & {\color[HTML]{6AA84F} \textbf{SFT}} & 30,27 & \textbf{36,80} \\  
\multirow{-4}{*}{\textbf{MEDICAL}} & {\color[HTML]{FF0000} \textbf{CPT+SFT}} & 31,60 & \textbf{36,53} \\ \hline
\multicolumn{4}{c}{\cellcolor[HTML]{CFE2F3}\textit{\textbf{Llama-13B}}} \\ \hline
 & \textbf{Base} & 25,51 & \textbf{34,83} \\  
 & {\color[HTML]{0000FF} \textbf{CPT}} & 26,64 & \textbf{37,21} \\  
 & {\color[HTML]{6AA84F} \textbf{SFT}} & 30,18 & \textbf{43,22} \\  
\multirow{-4}{*}{\textbf{GENERAL}} & {\color[HTML]{FF0000} \textbf{CPT+SFT}} & 31,41 & \textbf{43,62} \\ \hline
 & \textbf{Base} & 21,68 & \textbf{23,60} \\  
 & {\color[HTML]{0000FF} \textbf{CPT}} & 24,57 & \textbf{24,85} \\  
 & {\color[HTML]{6AA84F} \textbf{SFT}} & 30,10 & \textbf{46,99} \\  
\multirow{-4}{*}{\textbf{INSTRUCT}} & {\color[HTML]{FF0000} \textbf{CPT+SFT}} & 31,51 & \textbf{46,57} \\ \hline
 & \textbf{Base} & 23,97 & \textbf{24,28} \\  
 & {\color[HTML]{0000FF} \textbf{CPT}} & 23,37 & \textbf{30,87} \\  
 & {\color[HTML]{6AA84F} \textbf{SFT}} & 29,88 & \textbf{37,71} \\  
\multirow{-4}{*}{\textbf{MEDICAL}} & {\color[HTML]{FF0000} \textbf{CPT+SFT}} & 31,32 & \textbf{42,73} \\ \hline
\end{tabular}%
}
\caption{}
\label{tab:en-eval-results}
\end{table}

==> main-results-greedy.tex <==
% ---- Table ----
\begin{table*}[!t]
\centering
\begingroup
\setlength{\tabcolsep}{2.5pt}
\renewcommand{\arraystretch}{0.78}
\footnotesize

\scalebox{0.92}{
\begin{tabular}{ll S S S S}
\toprule
\multirow{2}{*}{\textbf{Model Type}} &
\multirow{2}{*}{\textbf{Strategy}} &
\multicolumn{2}{c}{\textbf{MCQ}} &
\textbf{MCQU} &
\textbf{Aggregation} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}
& &
{\textbf{EM}} & {\textbf{Hamming}} &
{\textbf{EM}} &
{\textbf{EM}} \\
\midrule

% ===================== Gemma-4B =====================
\multicolumn{6}{c}{\cellcolor[HTML]{CFE2F3}\textbf{Gemma-4B}}\\ \hline
\multirow{4}{*}{\textbf{GENERAL}}
 & Base    & 0.56 & 5.15  & 5.88  & 3.22 \\
 & {\color[HTML]{0000FF}CPT}     & 0.03 & 0.68  & 8.53  & 4.28 \\
 & {\color[HTML]{6AA84F}SFT}     & \textbf{1.73} & \textbf{19.48} & \textbf{19.81} & \textbf{10.77} \\
 & {\color[HTML]{FF0000}CPT+SFT} & 1.67 & 15.34 & 19.52 & 10.60 \\
\midrule
\multirow{4}{*}{\textbf{INSTRUCT}}
 & Base    & \uline{\textbf{6.81}} & \uline{\textbf{40.75}} & 28.88 & \uline{\textbf{17.85}} \\
 & {\color[HTML]{0000FF}CPT}     & 0.07 & 1.72  & 1.37  & 0.72 \\
 & {\color[HTML]{6AA84F}SFT}     & 1.38 & 10.17 & \uline{\textbf{31.87}} & 16.63 \\
 & {\color[HTML]{FF0000}CPT+SFT} & 1.22 & 8.61  & 30.66 & 15.94 \\
\midrule
\multirow{4}{*}{\textbf{MEDICAL}}
 & Base    & 1.22 & 11.28 & 11.47 & 6.34 \\
 & {\color[HTML]{0000FF}CPT}     & 1.62 & \textbf{18.11} & 11.18 & 6.40 \\
 & {\color[HTML]{6AA84F}SFT}     & 1.15 & 11.51 & \textbf{17.91} & 9.53 \\
 & {\color[HTML]{FF0000}CPT+SFT} & \textbf{1.67} & 16.54 & 17.63 & \textbf{9.65} \\

% ===================== Mistral-7B =====================
\midrule
\multicolumn{6}{c}{\cellcolor[HTML]{CFE2F3}\textbf{Mistral-7B}}\\ \hline
\multirow{4}{*}{\textbf{GENERAL}}
 & Base    & 0.15 & 2.90  & 4.04  & 2.09 \\
 & {\color[HTML]{0000FF}CPT}     & 0.44 & 3.75  & 13.71 & 7.07 \\
 & {\color[HTML]{6AA84F}SFT}     & \textbf{1.79} & \textbf{20.62} & \textbf{19.88} & \textbf{10.84} \\
 & {\color[HTML]{FF0000}CPT+SFT} & 1.42 & 17.95 & 19.57 & 10.49 \\
\midrule
\multirow{4}{*}{\textbf{INSTRUCT}}
 & Base    & 3.42 & 26.94 & 21.46 & 12.44 \\
 & {\color[HTML]{0000FF}CPT}     & 4.10 & 29.16 & 27.63 & 15.87 \\
 & {\color[HTML]{6AA84F}SFT}     & \uline{\textbf{11.94}} & \uline{\textbf{47.39}} & \uline{\textbf{31.52}} & \uline{\textbf{21.73}} \\
 & {\color[HTML]{FF0000}CPT+SFT} & 1.85 & 17.56 & 29.84 & 15.85 \\
\midrule
\multirow{4}{*}{\textbf{MEDICAL}}
 & Base    & 2.24 & 19.09 & 13.39 & 7.81 \\
 & {\color[HTML]{0000FF}CPT}     & \textbf{2.25} & 18.39 & 12.19 & 7.22 \\
 & {\color[HTML]{6AA84F}SFT}     & 1.95 & \textbf{20.68} & 18.47 & 10.21 \\
 & {\color[HTML]{FF0000}CPT+SFT} & 1.44 & 16.43 & \textbf{19.33} & \textbf{10.38} \\

% ===================== LLaMA-7B =====================
\midrule
\multicolumn{6}{c}{\cellcolor[HTML]{CFE2F3}\textbf{LLaMA-7B}}\\ \hline
\multirow{4}{*}{\textbf{GENERAL}}
 & Base    & 0.17 & 2.69  & 9.46  & 4.82 \\
 & {\color[HTML]{0000FF}CPT}     & 1.13 & 10.16 & 5.83  & 3.48 \\
 & {\color[HTML]{6AA84F}SFT}     & \textbf{1.82} & \textbf{24.64} & 16.08 & 8.95 \\
 & {\color[HTML]{FF0000}CPT+SFT} & 1.61 & 17.50 & \textbf{17.11} & \textbf{9.36} \\
\midrule
\multirow{4}{*}{\textbf{INSTRUCT}}
 & Base    & 0.03 & 0.64  & 0.04  & 0.03 \\
 & {\color[HTML]{0000FF}CPT}     & 4.92 & 40.87 & 0.04  & 2.48 \\
 & {\color[HTML]{6AA84F}SFT}     & \uline{\textbf{7.72}} & \uline{\textbf{42.70}} & \uline{\textbf{29.26}} & \uline{\textbf{18.49}} \\
 & {\color[HTML]{FF0000}CPT+SFT} & 1.03 & 6.36  & 0.07  & 0.55 \\
\midrule
\multirow{4}{*}{\textbf{MEDICAL}}
 & Base    & 0.14 & 1.98  & 0.57  & 0.35 \\
 & {\color[HTML]{0000FF}CPT}     & \textbf{2.11} & \textbf{24.01} & 12.20 & 7.16 \\
 & {\color[HTML]{6AA84F}SFT}     & 1.12 & 20.40 & 17.49 & 9.30 \\
 & {\color[HTML]{FF0000}CPT+SFT} & 1.67 & 15.87 & \textbf{18.29} & \textbf{9.98} \\

% ===================== LLaMA-13B =====================
\midrule
\multicolumn{6}{c}{\cellcolor[HTML]{CFE2F3}\textbf{LLaMA-13B}}\\ \hline
\multirow{4}{*}{\textbf{GENERAL}}
 & Base    & 0.29 & 0.84  & 11.77 & 6.03 \\
 & {\color[HTML]{0000FF}CPT}     & \textbf{2.81} & 21.03 & 10.49 & 6.65 \\
 & {\color[HTML]{6AA84F}SFT}     & 2.18 & 17.08 & 18.67 & 10.42 \\
 & {\color[HTML]{FF0000}CPT+SFT} & 1.65 & \textbf{21.56} & \textbf{19.84} & \textbf{10.74} \\
\midrule
\multirow{4}{*}{\textbf{INSTRUCT}}
 & Base    & 0.00 & 4.87  & 0.04  & 0.02 \\
 & {\color[HTML]{0000FF}CPT}     & 4.82 & 34.09 & 0.04  & 2.43 \\
 & {\color[HTML]{6AA84F}SFT}     & 10.92 & 42.98 & 30.13 & 20.53 \\
 & {\color[HTML]{FF0000}CPT+SFT} & \uline{\textbf{12.57}} & \uline{\textbf{44.02}} & \uline{\textbf{31.48}} & \uline{\textbf{22.02}} \\
\midrule
\multirow{4}{*}{\textbf{MEDICAL}}
 & Base    & 0.56 & 9.41  & 11.01 & 5.78 \\
 & {\color[HTML]{0000FF}CPT}     & 2.02 & \textbf{22.25} & 11.28 & 6.65 \\
 & {\color[HTML]{6AA84F}SFT}     & \textbf{2.07} & 21.50 & 18.11 & 10.09 \\
 & {\color[HTML]{FF0000}CPT+SFT} & 1.61 & 17.64 & \textbf{19.75} & \textbf{10.68} \\

\bottomrule
\end{tabular}
}
\caption{Greedy decoding results for MCQ and MCQU across model families and adaptation strategies.\textbf{Bold} denotes the best strategy and \uline{underlining} the best initialization.}
\label{tab:greedy-results}
\endgroup
\end{table*}


==> main-results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|cccc|ccc|}
\hline
 &  & \multicolumn{2}{c}{\textit{\textbf{QCM}}} & \textit{\textbf{QCMU}} & \textit{\textbf{Aggregation}} & \multicolumn{3}{c|}{\textbf{OEQA}} \\ \cline{3-9} 
\multirow{-2}{*}{\textbf{Model Type}} & \multirow{-2}{*}{\textbf{Strategy}} & \textbf{EM} & \textbf{Hamming} & \textbf{EM} & \textbf{EM} & \textit{\textbf{Rouge-L}} & \textit{\textbf{BERTScore-F1}} & \textit{\textbf{LLM-as-a-Judge}} \\ \hline
\multicolumn{9}{c}{\cellcolor[HTML]{CFE2F3}\textit{\textbf{Gemma-4B}}} \\ \hline 
 & \textbf{Base} & 2,24 & 30,17 & 27,11 & 14,68 & 7,11 & 46,62 & 25,09 \\ 
 & {\color[HTML]{0000FF} \textbf{CPT}} & 0,73 & 11,71 & 25,83 & 13,28 & \textbf{10,18} & \textbf{49,07} & \textbf{25,71} \\  
 & {\color[HTML]{6AA84F} \textbf{SFT}} & 3,73 & \textbf{43,57} & 32,36 & 18,05 & 8,23 & 47,76 & 21,60 \\  
\multirow{-4}{*}{\textbf{GENERAL}} & {\color[HTML]{FF0000} \textbf{CPT+SFT}} & \textbf{3,90} & 42,81 & \textbf{32,59} & \textbf{18,25} & 6,01 & 45,78 & 24,80 \\ \hline
 & \textbf{Base} & \textbf{4,83} & 44,01 & 29,30 & 17,06 & \textbf{7,38} & \textbf{48,94} & \textbf{47,71} \\  
 & {\color[HTML]{0000FF} \textbf{CPT}} & 3,47 & 46,00 & 25,05 & 14,26 & 4,57 & 42,77 & 13,35 \\  
 & {\color[HTML]{6AA84F} \textbf{SFT}} & 3,68 & \textbf{48,22} & \textbf{31,95} & \textbf{17,81} & 2,20 & 38,26 & 20,21 \\  
\multirow{-4}{*}{\textbf{INSTRUCT}} & {\color[HTML]{FF0000} \textbf{CPT+SFT}} & 3,42 & 48,14 & 30,73 & 17,07 & 3,12 & 40,90 & 20,76 \\ \hline
 & \textbf{Base} & 1,98 & 31,46 & 26,41 & 14,19 & \textbf{7,38} & \textbf{48,94} & \textbf{22,01} \\  
 & {\color[HTML]{0000FF} \textbf{CPT}} & 1,68 & 24,04 & 25,13 & 13,41 & 6,77 & 45,18 & 1,95 \\  
 & {\color[HTML]{6AA84F} \textbf{SFT}} & \textbf{3,54} & \textbf{46,22} & 30,66 & 17,10 & 5,70 & 45,66 & 14,23 \\  
\multirow{-4}{*}{\textbf{MEDICAL}} & {\color[HTML]{FF0000} \textbf{CPT+SFT}} & 3,38 & 43,28 & \textbf{30,86} & \textbf{17,12} & 5,04 & 43,05 & 11,41 \\ \hline
\multicolumn{9}{c}{\cellcolor[HTML]{CFE2F3}\textit{\textbf{Mistral-7B}}} \\ \hline
 & \textbf{Base} & 0,37 & 5,40 & 28,52 & 14,44 & 5,82 & 44,21 & \textbf{27,23} \\  
 & {\color[HTML]{0000FF} \textbf{CPT}} & 3,54 & 30,50 & 27,21 & 15,37 & 7,22 & 46,32 & 24,57 \\  
 & {\color[HTML]{6AA84F} \textbf{SFT}} & 5,24 & 21,62 & \textbf{32,88} & 19,06 & \textbf{8,83} & \textbf{48,02} & 22,93 \\  
\multirow{-4}{*}{\textbf{GENERAL}} & {\color[HTML]{FF0000} \textbf{CPT+SFT}} & \textbf{6,13} & \textbf{30,86} & 32,29 & \textbf{19,21} & 6,62 & 46,35 & 24,89 \\ \hline
 & \textbf{Base} & 4,86 & 23,53 & 24,92 & 14,89 & 7,34 & 49,66 & 30,14 \\  
 & {\color[HTML]{0000FF} \textbf{CPT}} & \textbf{7,32} & \textbf{36,18} & 28,79 & 18,06 & \textbf{13,51} & \textbf{53,87} & \textbf{37,59} \\  
 & {\color[HTML]{6AA84F} \textbf{SFT}} & 6,80 & 23,42 & \textbf{31,61} & \textbf{19,21} & 12,41 & 52,72 & 17,63 \\  
\multirow{-4}{*}{\textbf{INSTRUCT}} & {\color[HTML]{FF0000} \textbf{CPT+SFT}} & 5,45 & 32,47 & 30,09 & 17,77 & 9,02 & 48,99 & 32,13 \\ \hline
 & \textbf{Base} & 2,80 & 17,47 & 26,69 & 14,74 & 11,34 & \textbf{51,58} & 20,76 \\  
 & {\color[HTML]{0000FF} \textbf{CPT}} & 3,57 & 24,43 & 25,73 & 14,65 & \textbf{12,41} & 51,45 & 17,89 \\  
 & {\color[HTML]{6AA84F} \textbf{SFT}} & 3,36 & 26,37 & 31,62 & 17,49 & 8,75 & 47,86 & 16,72 \\  
\multirow{-4}{*}{\textbf{MEDICAL}} & {\color[HTML]{FF0000} \textbf{CPT+SFT}} & \textbf{4,94} & \textbf{27,27} & \textbf{32,58} & \textbf{18,76} & 9,15 & 48,63 & \textbf{24,96} \\ \hline
\multicolumn{9}{c}{\cellcolor[HTML]{CFE2F3}\textit{\textbf{Llama-7B}}} \\ \hline
 & \textbf{Base} & 1,33 & 12,01 & 25,72 & 13,53 & 5,05 & 41,27 & 9,39 \\  
 & {\color[HTML]{0000FF} \textbf{CPT}} & 1,12 & 12,86 & 25,59 & 13,36 & \textbf{10,58} & \textbf{47,85} & 3,78 \\  
 & {\color[HTML]{6AA84F} \textbf{SFT}} & 2,66 & 28,41 & 28,93 & 15,80 & 6,02 & 44,49 & 7,67 \\  
\multirow{-4}{*}{\textbf{GENERAL}} & {\color[HTML]{FF0000} \textbf{CPT+SFT}} & \textbf{3,17} & \textbf{46,00} & \textbf{29,89} & \textbf{16,53} & 5,85 & 44,67 & \textbf{12,26} \\ \hline
 & \textbf{Base} & 3,95 & 34,43 & 25,08 & 14,51 & 2,57 & 43,85 & 25,35 \\  
 & {\color[HTML]{0000FF} \textbf{CPT}} & 3,93 & \textbf{42,67} & 25,07 & 14,50 & 11,16 & \textbf{51,37} & 26,06 \\  
 & {\color[HTML]{6AA84F} \textbf{SFT}} & \textbf{5,12} & 21,06 & \textbf{29,32} & \textbf{17,22} & \textbf{11,44} & 51,28 & 12,92 \\  
\multirow{-4}{*}{\textbf{INSTRUCT}} & {\color[HTML]{FF0000} \textbf{CPT+SFT}} & 3,13 & 25,98 & 25,07 & 14,10 & 9,92 & 50,99 & \textbf{27,84} \\ \hline
 & \textbf{Base} & 0,23 & 2,90 & 24,43 & 12,33 & 5,61 & 43,25 & 12,50 \\  
 & {\color[HTML]{0000FF} \textbf{CPT}} & 2,37 & 28,06 & 25,60 & 13,99 & \textbf{8,00} & \textbf{45,79} & 13,14 \\  
 & {\color[HTML]{6AA84F} \textbf{SFT}} & 3,24 & 29,10 & 30,44 & 16,84 & 5,40 & 42,25 & 9,50 \\  
\multirow{-4}{*}{\textbf{MEDICAL}} & {\color[HTML]{FF0000} \textbf{CPT+SFT}} & \textbf{3,80} & \textbf{44,95} & \textbf{31,52} & \textbf{17,66} & 5,87 & 44,34 & \textbf{17,39} \\ \hline
\multicolumn{9}{c}{\cellcolor[HTML]{CFE2F3}\textit{\textbf{Llama-13B}}} \\ \hline
 & \textbf{Base} & 2,14 & 21,20 & 26,11 & 14,13 & 2,10 & 33,25 & 11,79 \\  
 & {\color[HTML]{0000FF} \textbf{CPT}} & 2,53 & 19,17 & 26,99 & 14,76 & \textbf{14,12} & \textbf{50,36} & 5,66 \\  
 & {\color[HTML]{6AA84F} \textbf{SFT}} & \textbf{3,54} & \textbf{40,49} & 30,95 & 17,24 & 5,60 & 43,19 & 14,88 \\  
\multirow{-4}{*}{\textbf{GENERAL}} & {\color[HTML]{FF0000} \textbf{CPT+SFT}} & 3,34 & 29,59 & \textbf{32,36} & \textbf{17,85} & 6,30 & 45,45 & \textbf{20,38} \\ \hline
 & \textbf{Base} & 0,09 & 29,74 & 21,52 & 10,81 & 3,40 & 45,31 & 30,02 \\  
 & {\color[HTML]{0000FF} \textbf{CPT}} & 5,63 & \textbf{37,40} & 25,01 & 15,32 & 12,34 & \textbf{53,07} & \textbf{36,19} \\  
 & {\color[HTML]{6AA84F} \textbf{SFT}} & 6,58 & 23,96 & 30,20 & 18,39 & 11,54 & 50,94 & 11,81 \\  
\multirow{-4}{*}{\textbf{INSTRUCT}} & {\color[HTML]{FF0000} \textbf{CPT+SFT}} & \textbf{7,77} & 25,26 & \textbf{31,58} & \textbf{19,68} & \textbf{12,86} & 52,46 & 20,22 \\ \hline
 & \textbf{Base} & 1,77 & 11,82 & 24,62 & 13,19 & 5,00 & 42,11 & 10,86 \\  
 & {\color[HTML]{0000FF} \textbf{CPT}} & 2,26 & 30,87 & 24,10 & 13,18 & 8,00 & 45,79 & 13,39 \\  
 & {\color[HTML]{6AA84F} \textbf{SFT}} & 3,12 & 41,24 & 30,62 & 16,87 & 6,85 & 45,22 & 13,77 \\  
\multirow{-4}{*}{\textbf{MEDICAL}} & {\color[HTML]{FF0000} \textbf{CPT+SFT}} & \textbf{3,24} & \textbf{45,59} & \textbf{32,25} & \textbf{17,74} & \textbf{8,38} & \textbf{46,29} & \textbf{19,55} \\ \hline
\end{tabular}%
}
\caption{}
\label{tab:main-results}
\end{table*}

==> mcqa-res.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[!t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{llllllllll}
                          &                        & \multicolumn{4}{l}{QCM}                                      & \multicolumn{2}{l}{QCMU} & \multicolumn{2}{l}{Aggregation} \\
                          & \multirow{2}{*}{Model} & \multicolumn{2}{l}{Greedy} & \multicolumn{2}{l}{Constrained} & Greedy    & Constrained  & Greedy       & Constrained      \\
                          &                        & EM           & Hamming     & EM             & Hamming        & \multicolumn{2}{l}{EM}   & \multicolumn{2}{l}{EM}          \\
                          & \multicolumn{9}{c}{GEMMA-4B FAMILY}                                                                                                                \\
\multirow{4}{*}{GENERAL}  & Base                   & 0,56\%       & 5,15\%      & 2,24\%         & 30,17\%        & 5,88\%    & 27,11\%      & 3,22\%       & 14,68\%          \\
                          & CPT                    & 0,03\%       & 0,68\%      & 0,73\%         & 11,71\%        & 8,53\%    & 25,83\%      & 4,28\%       & 13,28\%          \\
                          & SFT                    & 1,73\%       & 19,48\%     & 3,73\%         & 43,57\%        & 19,81\%   & 32,36\%      & 10,77\%      & 18,05\%          \\
                          & CPT+SFT                & 1,67\%       & 15,34\%     & 3,90\%         & 42,81\%        & 19,52\%   & 32,59\%      & 10,60\%      & 18,25\%          \\
\multirow{4}{*}{INSTRUCT} & Base                   & 6,81\%       & 40,75\%     & 4,83\%         & 44,01\%        & 28,88\%   & 29,30\%      & 17,85\%      & 17,06\%          \\
                          & CPT                    & 0,07\%       & 1,72\%      & 3,47\%         & 46,00\%        & 1,37\%    & 25,05\%      & 0,72\%       & 14,26\%          \\
                          & SFT                    & 1,38\%       & 10,17\%     & 3,68\%         & 48,22\%        & 31,87\%   & 31,95\%      & 16,63\%      & 17,81\%          \\
                          & CPT+SFT                & 1,22\%       & 8,61\%      & 3,42\%         & 48,14\%        & 30,66\%   & 30,73\%      & 15,94\%      & 17,07\%          \\
\multirow{4}{*}{MEDICAL}  & Base                   & 1,22\%       & 11,28\%     & 1,98\%         & 31,46\%        & 11,47\%   & 26,41\%      & 6,34\%       & 14,19\%          \\
                          & CPT                    & 1,62\%       & 18,11\%     & 1,68\%         & 24,04\%        & 11,18\%   & 25,13\%      & 6,40\%       & 13,41\%          \\
                          & SFT                    & 1,15\%       & 11,51\%     & 3,54\%         & 46,22\%        & 17,91\%   & 30,66\%      & 9,53\%       & 17,10\%          \\
                          & CPT+SFT                & 1,67\%       & 16,54\%     & 3,38\%         & 43,28\%        & 17,63\%   & 30,86\%      & 9,65\%       & 17,12\%          \\
                          & \multicolumn{9}{c}{Mistral-7B FAMILY}                                                                                                              \\
\multirow{4}{*}{GENERAL}  & Base                   & 0,15\%       & 2,90\%      & 0,37\%         & 5,40\%         & 4,04\%    & 28,52\%      & 2,09\%       & 14,44\%          \\
                          & CPT                    & 0,44\%       & 3,75\%      & 3,54\%         & 30,50\%        & 13,71\%   & 27,21\%      & 7,07\%       & 15,37\%          \\
                          & SFT                    & 1,79\%       & 20,62\%     & 5,24\%         & 21,62\%        & 19,88\%   & 32,88\%      & 10,84\%      & 19,06\%          \\
                          & CPT+SFT                & 1,42\%       & 17,95\%     & 6,13\%         & 30,86\%        & 19,57\%   & 32,29\%      & 10,49\%      & 19,21\%          \\
\multirow{4}{*}{INSTRUCT} & Base                   & 3,42\%       & 26,94\%     & 4,86\%         & 23,53\%        & 21,46\%   & 24,92\%      & 12,44\%      & 14,89\%          \\
                          & CPT                    & 4,10\%       & 29,16\%     & 7,32\%         & 36,18\%        & 27,63\%   & 28,79\%      & 15,87\%      & 18,06\%          \\
                          & SFT                    & 11,94\%      & 47,39\%     & 6,80\%         & 23,42\%        & 31,52\%   & 31,61\%      & 21,73\%      & 19,21\%          \\
                          & CPT+SFT                & 1,85\%       & 17,56\%     & 5,45\%         & 32,47\%        & 29,84\%   & 30,09\%      & 15,85\%      & 17,77\%          \\
\multirow{4}{*}{MEDICAL}  & Base                   & 2,24\%       & 19,09\%     & 2,80\%         & 17,47\%        & 13,39\%   & 26,69\%      & 7,81\%       & 14,74\%          \\
                          & CPT                    & 2,25\%       & 18,39\%     & 3,57\%         & 24,43\%        & 12,19\%   & 25,73\%      & 7,22\%       & 14,65\%          \\
                          & SFT                    & 1,95\%       & 20,68\%     & 3,36\%         & 26,37\%        & 18,47\%   & 31,62\%      & 10,21\%      & 17,49\%          \\
                          & CPT+SFT                & 1,44\%       & 16,43\%     & 4,94\%         & 27,27\%        & 19,33\%   & 32,58\%      & 10,38\%      & 18,76\%          \\
                          & \multicolumn{9}{c}{LLAMA-7B FAMILY}                                                                                                                \\
\multirow{4}{*}{GENERAL}  & Base                   & 0,17\%       & 2,69\%      & 1,33\%         & 12,01\%        & 9,46\%    & 25,72\%      & 4,82\%       & 13,53\%          \\
                          & CPT                    & 1,13\%       & 10,16\%     & 1,12\%         & 12,86\%        & 5,83\%    & 25,59\%      & 3,48\%       & 13,36\%          \\
                          & SFT                    & 1,82\%       & 24,64\%     & 2,66\%         & 28,41\%        & 16,08\%   & 28,93\%      & 8,95\%       & 15,80\%          \\
                          & CPT+SFT                & 1,61\%       & 17,50\%     & 3,17\%         & 46,00\%        & 17,11\%   & 29,89\%      & 9,36\%       & 16,53\%          \\
\multirow{4}{*}{INSTRUCT} & Base                   & 0,03\%       & 0,64\%      & 3,95\%         & 34,43\%        & 0,04\%    & 25,08\%      & 0,03\%       & 14,51\%          \\
                          & CPT                    & 4,92\%       & 40,87\%     & 3,93\%         & 42,67\%        & 0,04\%    & 25,07\%      & 2,48\%       & 14,50\%          \\
                          & SFT                    & 7,72\%       & 42,70\%     & 5,12\%         & 21,06\%        & 29,26\%   & 29,32\%      & 18,49\%      & 17,22\%          \\
                          & CPT+SFT                & 1,03\%       & 6,36\%      & 3,13\%         & 25,98\%        & 0,07\%    & 25,07\%      & 0,55\%       & 14,10\%          \\
\multirow{4}{*}{MEDICAL}  & Base                   & 0,14\%       & 1,98\%      & 0,23\%         & 2,90\%         & 0,57\%    & 24,43\%      & 0,35\%       & 12,33\%          \\
                          & CPT                    & 2,11\%       & 24,01\%     & 2,37\%         & 28,06\%        & 12,20\%   & 25,60\%      & 7,16\%       & 13,99\%          \\
                          & SFT                    & 1,12\%       & 20,40\%     & 3,24\%         & 29,10\%        & 17,49\%   & 30,44\%      & 9,30\%       & 16,84\%          \\
                          & CPT+SFT                & 1,67\%       & 15,87\%     & 3,80\%         & 44,95\%        & 18,29\%   & 31,52\%      & 9,98\%       & 17,66\%          \\
                          & \multicolumn{9}{c}{LLAMA-13B FAMILY}                                                                                                               \\
\multirow{4}{*}{GENERAL}  & Base                   & 0,29\%       & 0,84\%      & 2,14\%         & 21,20\%        & 11,77\%   & 26,11\%      & 6,03\%       & 14,13\%          \\
                          & CPT                    & 2,81\%       & 21,03\%     & 2,53\%         & 19,17\%        & 10,49\%   & 26,99\%      & 6,65\%       & 14,76\%          \\
                          & SFT                    & 2,18\%       & 17,08\%     & 3,54\%         & 40,49\%        & 18,67\%   & 30,95\%      & 10,42\%      & 17,24\%          \\
                          & CPT+SFT                & 1,65\%       & 21,56\%     & 3,34\%         & 29,59\%        & 19,84\%   & 32,36\%      & 10,74\%      & 17,85\%          \\
\multirow{4}{*}{INSTRUCT} & Base                   & 0,00\%       & 4,87\%      & 0,09\%         & 29,74\%        & 0,04\%    & 21,52\%      & 0,02\%       & 10,81\%          \\
                          & CPT                    & 4,82\%       & 34,09\%     & 5,63\%         & 37,40\%        & 0,04\%    & 25,01\%      & 2,43\%       & 15,32\%          \\
                          & SFT                    & 10,92\%      & 42,98\%     & 6,58\%         & 23,96\%        & 30,13\%   & 30,20\%      & 20,53\%      & 18,39\%          \\
                          & CPT+SFT                & 12,57\%      & 44,02\%     & 7,77\%         & 25,26\%        & 31,48\%   & 31,58\%      & 22,02\%      & 19,68\%          \\
\multirow{4}{*}{MEDICAL}  & Base                   & 0,56\%       & 9,41\%      & 1,77\%         & 11,82\%        & 11,01\%   & 24,62\%      & 5,78\%       & 13,19\%          \\
                          & CPT                    & 2,02\%       & 22,25\%     & 2,26\%         & 30,87\%        & 11,28\%   & 24,10\%      & 6,65\%       & 13,18\%          \\
                          & SFT                    & 2,07\%       & 21,50\%     & 3,12\%         & 41,24\%        & 18,11\%   & 30,62\%      & 10,09\%      & 16,87\%          \\
                          & CPT+SFT                & 1,61\%       & 17,64\%     & 3,24\%         & 45,59\%        & 19,75\%   & 32,25\%      & 10,68\%      & 17,74\%         
\end{tabular}%
}
\caption{MCQA performance (\%) across model families and adaptation strategies. We report Exact Match (EM) and Hamming scores for QCM and QCMU under greedy and constrained decoding, along with aggregated results.}
\label{tab:MCQA-main-res}
\end{table*}

